Wire-Cell 3D Pattern Recognition Techniques for Neutrino Event Reconstruction in Large LArTPCs: Algorithm Description and Quantitative Evaluation with MicroBooNE Simulation

Wire-Cell is a 3D event reconstruction package for liquid argon time projection chambers. Through geometry, time, and drifted charge from multiple readout wire planes, 3D space points with associated charge are reconstructed prior to the pattern recognition stage. Pattern recognition techniques, including track trajectory and $dQ/dx$ (ionization charge per unit length) fitting, 3D neutrino vertex fitting, track and shower separation, particle-level clustering, and particle identification are then applied on these 3D space points as well as the original 2D projection measurements. A deep neural network is developed to enhance the reconstruction of the neutrino interaction vertex. Compared to traditional algorithms, the deep neural network boosts the vertex efficiency by a relative 30\% for charged-current $\nu_e$ interactions. This pattern recognition achieves 80-90\% reconstruction efficiencies for primary leptons, after a 65.8\% (72.9\%) vertex efficiency for charged-current $\nu_e$ ($\nu_\mu$) interactions. Based on the resulting reconstructed particles and their kinematics, we also achieve 15-20\% energy reconstruction resolutions for charged-current neutrino interactions.

==> microboone-author-list-sept2020-PRD-WC-reco.tex <==
% ****** Start of file apssamp.tex ******
% See the REVTeX 4 README file
%
%%\documentclass[aps,prd,twocolumn,showpacs,superscriptaddress]{revtex4}  
%%\usepackage{graphicx}% Include figure files
%%\usepackage{dcolumn}% Align table columns on decimal point
%%\usepackage{bm}% bold math

% Jan 2019 notes:
% invited author for CC pi0: H. Chen (as per IB vote, first PRL)
% invited author for CC inclusive and any papers using MCS: Polina Abratenko 

%%\begin{document}
%\title{MicroBooNE Author List - September 2020 (PRD Format)}
%%\title{MicroBooNE Author List - September 2020 - special author list for WC PRL (PRL Format)}

%%\title{MicroBooNE Author List - July 2020 -- special version for CCNp paper (PRD Format)}

% List of institutions in command form:
\newcommand{\Bern}{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\newcommand{\BNL}{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\newcommand{\UCSB}{University of California, Santa Barbara, CA, 93106, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\StKates}{St. Catherine University, Saint Paul, MN 55105, USA}
\newcommand{\CIEMAT}{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid E-28040, Spain}
\newcommand{\Chicago}{University of Chicago, Chicago, IL, 60637, USA}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, 45221, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY, 10027, USA}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\newcommand{\Granada}{Universidad de Granada, Granada E-18071, Spain}
\newcommand{\Harvard}{Harvard University, Cambridge, MA 02138, USA}
\newcommand{\IIT}{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\newcommand{\KSU}{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\newcommand{\Manchester}{The University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\MIT}{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI, 48109, USA}
\newcommand{\Minnesota}{University of Minnesota, Minneapolis, MN, 55455, USA}
\newcommand{\NMSU}{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\newcommand{\Otterbein}{Otterbein University, Westerville, OH, 43081, USA}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\PNNL}{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, 08854, USA}
\newcommand{\StMarys}{Saint Mary's University of Minnesota, Winona, MN, 55987, USA}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology (SDSMT), Rapid City, SD, 57701, USA}
\newcommand{\Maine}{University of Southern Maine, Portland, ME, 04104, USA}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY, 13244, USA}
\newcommand{\TelAviv}{Tel Aviv University, Tel Aviv, Israel, 69978}
\newcommand{\Tennessee}{University of Tennessee, Knoxville, TN, 37996, USA}
\newcommand{\UTA}{University of Texas, Arlington, TX, 76019, USA}
\newcommand{\Tufts}{Tufts University, Medford, MA, 02155, USA}
\newcommand{\VTech}{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\newcommand{\Warwick}{University of Warwick, Coventry CV4 7AL, United Kingdom}
\newcommand{\Yale}{Wright Laboratory, Department of Physics, Yale University, New Haven, CT, 06520, USA}
%%\newcommand{\listerThanks}{Now at University of Wisconsin, Madison}

% So that institutions appear in alphabetical order:
\affiliation{\Bern}
\affiliation{\BNL}
\affiliation{\UCSB}
\affiliation{\Cambridge}
\affiliation{\StKates}
\affiliation{\CIEMAT}
\affiliation{\Chicago}
\affiliation{\Cincinnati}
\affiliation{\CSU}
\affiliation{\Columbia}
\affiliation{\FNAL}
\affiliation{\Granada}
\affiliation{\Harvard}
\affiliation{\IIT}
\affiliation{\KSU}
\affiliation{\Lancaster}
\affiliation{\LANL}
\affiliation{\Manchester}
\affiliation{\MIT}
\affiliation{\Michigan}
\affiliation{\Minnesota}
\affiliation{\NMSU}
\affiliation{\Otterbein}
\affiliation{\Oxford}
\affiliation{\PNNL}
\affiliation{\Pitt}
\affiliation{\Rutgers}
\affiliation{\StMarys}
\affiliation{\SLAC}
\affiliation{\SDSMT}
\affiliation{\Maine}
\affiliation{\Syracuse}
\affiliation{\TelAviv}
\affiliation{\Tennessee}
\affiliation{\UTA}
\affiliation{\Tufts}
\affiliation{\VTech}
\affiliation{\Warwick}
\affiliation{\Yale}

% Authors in alphabetical order
%\author{P.~Abratenko} \affiliation{\Michigan} % for CC incl and any papers using MCS
\author{P.~Abratenko} \affiliation{\Tufts} 
\author{M.~Alrashed} \affiliation{\KSU}
\author{R.~An} \affiliation{\IIT}
\author{J.~Anthony} \affiliation{\Cambridge}
\author{J.~Asaadi} \affiliation{\UTA}
\author{A.~Ashkenazi} \affiliation{\MIT}
\author{S.~Balasubramanian} \affiliation{\Yale}
\author{B.~Baller} \affiliation{\FNAL}
\author{C.~Barnes} \affiliation{\Michigan}
\author{G.~Barr} \affiliation{\Oxford}
\author{V.~Basque} \affiliation{\Manchester}
\author{L.~Bathe-Peters} \affiliation{\Harvard}
\author{O.~Benevides~Rodrigues} \affiliation{\Syracuse}
\author{S.~Berkman} \affiliation{\FNAL}
\author{A.~Bhanderi} \affiliation{\Manchester}
\author{A.~Bhat} \affiliation{\Syracuse}
\author{M.~Bishai} \affiliation{\BNL}
\author{A.~Blake} \affiliation{\Lancaster}
\author{T.~Bolton} \affiliation{\KSU}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{D.~Caratelli} \affiliation{\FNAL}
\author{I.~Caro~Terrazas} \affiliation{\CSU}
\author{R.~Castillo~Fernandez} \affiliation{\FNAL}
\author{F.~Cavanna} \affiliation{\FNAL}
\author{G.~Cerati} \affiliation{\FNAL}
%\author{H.~Chen} \affiliation{\BNL}  % for CC pi0 only
\author{Y.~Chen} \affiliation{\Bern}
\author{E.~Church} \affiliation{\PNNL}
\author{D.~Cianci} \affiliation{\Columbia}
\author{J.~M.~Conrad} \affiliation{\MIT}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Cooper-Troendle} \affiliation{\Yale}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\Columbia}\affiliation{\CIEMAT}
\author{M.~Del~Tutto} \affiliation{\FNAL}
\author{D.~Devitt} \affiliation{\Lancaster}
\author{R.~Diurba}\affiliation{\Minnesota}
\author{L.~Domine} \affiliation{\SLAC}
\author{R.~Dorrill} \affiliation{\IIT}
\author{K.~Duffy} \affiliation{\FNAL}
\author{S.~Dytman} \affiliation{\Pitt}
\author{B.~Eberly} \affiliation{\Maine}
\author{A.~Ereditato} \affiliation{\Bern}
\author{L.~Escudero~Sanchez} \affiliation{\Cambridge}
\author{J.~J.~Evans} \affiliation{\Manchester}
\author{G.~A.~Fiorentini~Aguirre} \affiliation{\SDSMT}
\author{R.~S.~Fitzpatrick} \affiliation{\Michigan}
\author{B.~T.~Fleming} \affiliation{\Yale}
\author{N.~Foppiani} \affiliation{\Harvard}
\author{D.~Franco} \affiliation{\Yale}
\author{A.~P.~Furmanski}\affiliation{\Minnesota}
\author{D.~Garcia-Gamez} \affiliation{\Granada}
\author{S.~Gardiner} \affiliation{\FNAL}
\author{G.~Ge} \affiliation{\Columbia}
\author{S.~Gollapinni} \affiliation{\Tennessee}\affiliation{\LANL}
\author{O.~Goodwin} \affiliation{\Manchester}
\author{E.~Gramellini} \affiliation{\FNAL}
\author{P.~Green} \affiliation{\Manchester}
\author{H.~Greenlee} \affiliation{\FNAL}
\author{W.~Gu} \affiliation{\BNL}
\author{R.~Guenette} \affiliation{\Harvard}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{L.~Hagaman} \affiliation{\Yale}
\author{E.~Hall} \affiliation{\MIT}
\author{P.~Hamilton} \affiliation{\Syracuse}
\author{O.~Hen} \affiliation{\MIT}
\author{G.~A.~Horton-Smith} \affiliation{\KSU}
\author{A.~Hourlier} \affiliation{\MIT}
\author{E.-C.~Huang} \affiliation{\LANL}
\author{R.~Itay} \affiliation{\SLAC}
\author{C.~James} \affiliation{\FNAL}
\author{J.~Jan~de~Vries} \affiliation{\Cambridge}
\author{X.~Ji} \affiliation{\BNL}
\author{L.~Jiang} \affiliation{\VTech}
\author{J.~H.~Jo} \affiliation{\Yale}
\author{R.~A.~Johnson} \affiliation{\Cincinnati}
\author{Y.-J.~Jwa} \affiliation{\Columbia}
\author{N.~Kamp} \affiliation{\MIT}
\author{N.~Kaneshige} \affiliation{\UCSB}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{W.~Ketchum} \affiliation{\FNAL}
\author{B.~Kirby} \affiliation{\BNL}
\author{M.~Kirby} \affiliation{\FNAL}
\author{T.~Kobilarcik} \affiliation{\FNAL}
\author{I.~Kreslo} \affiliation{\Bern}
\author{R.~LaZur} \affiliation{\CSU}
\author{I.~Lepetic} \affiliation{\Rutgers}
\author{K.~Li} \affiliation{\Yale}
\author{Y.~Li} \affiliation{\BNL}
%%\author{A.~Lister}\thanks{\listerThanks} \affiliation{\Lancaster}  % special for CC Np paper
\author{B.~R.~Littlejohn} \affiliation{\IIT}
\author{D.~Lorca} \affiliation{\Bern}
\author{W.~C.~Louis} \affiliation{\LANL}
\author{X.~Luo} \affiliation{\UCSB}
\author{A.~Marchionni} \affiliation{\FNAL}
\author{C.~Mariani} \affiliation{\VTech}
\author{D.~Marsden} \affiliation{\Manchester}
\author{J.~Marshall} \affiliation{\Warwick}
\author{J.~Martin-Albo} \affiliation{\Harvard}
\author{D.~A.~Martinez~Caicedo} \affiliation{\SDSMT}
\author{K.~Mason} \affiliation{\Tufts}
\author{A.~Mastbaum} \affiliation{\Rutgers}
\author{N.~McConkey} \affiliation{\Manchester}
\author{V.~Meddage} \affiliation{\KSU}
\author{T.~Mettler}  \affiliation{\Bern}
\author{K.~Miller} \affiliation{\Chicago}
\author{J.~Mills} \affiliation{\Tufts}
\author{K.~Mistry} \affiliation{\Manchester}
\author{A.~Mogan} \affiliation{\Tennessee}
\author{T.~Mohayai} \affiliation{\FNAL}
\author{J.~Moon} \affiliation{\MIT}
\author{M.~Mooney} \affiliation{\CSU}
\author{A.~F.~Moor} \affiliation{\Cambridge}
\author{C.~D.~Moore} \affiliation{\FNAL}
\author{L.~Mora~Lepin} \affiliation{\Manchester}
\author{J.~Mousseau} \affiliation{\Michigan}
\author{M.~Murphy} \affiliation{\VTech}
\author{D.~Naples} \affiliation{\Pitt}
\author{A.~Navrer-Agasson} \affiliation{\Manchester}
\author{R.~K.~Neely} \affiliation{\KSU}
\author{P.~Nienaber} \affiliation{\StMarys}
\author{J.~Nowak} \affiliation{\Lancaster}
\author{O.~Palamara} \affiliation{\FNAL}
\author{V.~Paolone} \affiliation{\Pitt}
\author{A.~Papadopoulou} \affiliation{\MIT}
\author{V.~Papavassiliou} \affiliation{\NMSU}
\author{S.~F.~Pate} \affiliation{\NMSU}
\author{A.~Paudel} \affiliation{\KSU}
\author{Z.~Pavlovic} \affiliation{\FNAL}
\author{E.~Piasetzky} \affiliation{\TelAviv}
\author{I.~D.~Ponce-Pinto} \affiliation{\Columbia}
\author{D.~Porzio} \affiliation{\Manchester}
\author{S.~Prince} \affiliation{\Harvard}
\author{X.~Qian} \affiliation{\BNL}
\author{J.~L.~Raaf} \affiliation{\FNAL}
\author{V.~Radeka} \affiliation{\BNL}
\author{A.~Rafique} \affiliation{\KSU}
\author{M.~Reggiani-Guzzo} \affiliation{\Manchester}
\author{L.~Ren} \affiliation{\NMSU}
\author{L.~Rochester} \affiliation{\SLAC}
\author{J.~Rodriguez Rondon} \affiliation{\SDSMT}
\author{H.~E.~Rogers}\affiliation{\StKates}
\author{M.~Rosenberg} \affiliation{\Pitt}
\author{M.~Ross-Lonergan} \affiliation{\Columbia}
\author{B.~Russell} \affiliation{\Yale}
\author{G.~Scanavini} \affiliation{\Yale}
\author{D.~W.~Schmitz} \affiliation{\Chicago}
\author{A.~Schukraft} \affiliation{\FNAL}
\author{W.~Seligman} \affiliation{\Columbia}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{R.~Sharankova} \affiliation{\Tufts}
\author{J.~Sinclair} \affiliation{\Bern}
\author{A.~Smith} \affiliation{\Cambridge}
\author{E.~L.~Snider} \affiliation{\FNAL}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{S.~S{\"o}ldner-Rembold} \affiliation{\Manchester}
\author{S.~R.~Soleti} \affiliation{\Oxford}\affiliation{\Harvard}
\author{P.~Spentzouris} \affiliation{\FNAL}
\author{J.~Spitz} \affiliation{\Michigan}
\author{M.~Stancari} \affiliation{\FNAL}
\author{J.~St.~John} \affiliation{\FNAL}
\author{T.~Strauss} \affiliation{\FNAL}
\author{K.~Sutton} \affiliation{\Columbia}
\author{S.~Sword-Fehlberg} \affiliation{\NMSU}
\author{A.~M.~Szelc} \affiliation{\Manchester}
\author{N.~Tagg} \affiliation{\Otterbein}
\author{W.~Tang} \affiliation{\Tennessee}
\author{K.~Terao} \affiliation{\SLAC}
\author{C.~Thorpe} \affiliation{\Lancaster}
\author{M.~Toups} \affiliation{\FNAL}
\author{Y.-T.~Tsai} \affiliation{\SLAC}
\author{S.~Tufanli} \affiliation{\Yale}
\author{M.~A.~Uchida} \affiliation{\Cambridge}
\author{T.~Usher} \affiliation{\SLAC}
\author{W.~Van~De~Pontseele} \affiliation{\Oxford}\affiliation{\Harvard}
\author{B.~Viren} \affiliation{\BNL}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\BNL}
\author{Z.~Williams} \affiliation{\UTA}
\author{S.~Wolbers} \affiliation{\FNAL}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{M.~Wospakrik} \affiliation{\FNAL}
\author{W.~Wu} \affiliation{\FNAL}
\author{E.~Yandel} \affiliation{\UCSB}
\author{T.~Yang} \affiliation{\FNAL}
\author{G.~Yarbrough} \affiliation{\Tennessee}
\author{L.~E.~Yates} \affiliation{\MIT}
\author{H.~W.~Yu} \affiliation{\BNL}  % special for WC PRL
\author{G.~P.~Zeller} \affiliation{\FNAL}
\author{J.~Zennamo} \affiliation{\FNAL}
\author{C.~Zhang} \affiliation{\BNL}

\collaboration{The MicroBooNE Collaboration}
\emailAdd{microboone\_info@fnal.gov}\noaffiliation


%%\maketitle

%%\end{document}



